Sampling with a Black Box: Faster Parameterized Approximation Algorithms for Vertex Deletion Problems

In this paper we introduce Sampling with a Black Box, a generic technique for the design of parameterized approximation algorithms for vertex deletion problems (e.g., Vertex Cover, Feedback Vertex Set, etc.). The technique relies on two components: $\bullet$ A Sampling Step. A polynomial time randomized algorithm which given a graph $G$ returns a random vertex $v$ such that the optimum of $G\setminus \{v\}$ is smaller by $1$ than the optimum of $G$ with some prescribed probability $q$. We show such algorithms exists for multiple vertex deletion problems. $\bullet$ A Black Box algorithm which is either an exact parameterized algorithm or a polynomial time approximation algorithm. Our technique combines these two components together. The sampling step is applied iteratively to remove vertices from the input graph, and then the solution is extended using the black box algorithm. The process is repeated sufficiently many times so that the target approximation ratio is attained with a constant probability. The main novelty of our work lies in the analysis of the framework and the optimization of the parameters it uses. We use the technique to derive parameterized approximation algorithm for several vertex deletion problems, including Feedback Vertex Set, $d$-Hitting Set and $\ell$-Path Vertex Cover. In particular, for every approximation ratio $1<\beta<2$, we attain a parameterized $\beta$-approximation for Feedback Vertex Set which is faster than the parameterized $\beta$-approximation of [Jana, Lokshtanov, Mandal, Rai and Saurabh, MFCS 23']. Furthermore, our algorithms are always faster than the algorithms attained using Fidelity Preserving Transformations [Fellows, Kulik, Rosamond, and Shachnai, JCSS 18'].

==> advanced.tex <==

\subsection{Branching Steps and the Generic Algorithm}
Let $\cG$ be a family of hyper graphs and let $\Pi$ be a polynomial time decidable hyper graph property. Throughout this section we use the notation $\cG$ and $\Pi$ for a generic family of hypergraphs and property.
 We use $\OPT_{\cG,\Pi}(G)$ to denote the size of an optimal solution for $G\in \cG$ with respect to the $\gpivd$ problem. That is, $\OPT_{\cG,\Pi}(G) = \min\left\{ \abs{S}\,\middle|\,S\subseteq V(G) \textnormal{ and } G\setminus S \in \Pi\right\}$.  If $\cG$ and $\Pi$ are known by context we use $\OPT$ instead of $\OPT_{\cG,\Pi}$. 
 
We use  \texttt{Vertex Cover}  as a running example throughout the section. The problem is the $\svcvd$ problem in which $\vcG$ is the set of all (standard) graphs and $\vcPi$ is the set of all graphs with no edges. Alternatively, using the notations of \Cref{sec:forbidden} we can define $\vcPi=\Pi^{\{F\}}$ where $F=(\{1,2\}, \{(1,2)\})$ is a graph of a two vertices and an edge connecting them.  

We use an abstract notion of branching step. We rely on it to define $\proc{\delta}{p}$s for various problems in a generic way.
\begin{definition}
	\label{def:step}
A {\em branching step}  for $\gpivd$ is a deterministic polynomial time algorithm whose input is a graph $G\in \cG\setminus \Pi$ and a number $x\in [0,1]$ (which serves as a source of randomness), and returns a non-empty $S\subseteq V[G]$.
\end{definition}
We note that we define branching step as a {\em deterministic} algorithm which receive a value $x\in[0,1]$ as part of its input. This value is seen by the algorithm as a random variable with a uniform distribution on the interval $[0,1]$. This will later allow us to track dependencies (and independencies) in the execution of our generic procedure. The requirements in \Cref{def:step} are minimalist. We later describe additional properties of branching steps that will be needed to achieve lower bound the success probability of the generic procedure

\begin{algorithm}
	\begin{algorithmic}[1]
		\Configuration $\gamma\in (0,1)$
		\Input graph $G \in \vcG\setminus \vcPi$, number $x\in [0,1]$ 
		\If {there is $v\in V[G]$ with $\deg_{G}(v)\geq 3$\label{simple:v}} 
		\State let $N$ be $3$ of the neighbors of $v$ \label{simple:N}
		\State {\bf if} $x\leq \gamma$  {\bf then return} $\{v\}$ {\bf else return }N   
		\label{simple:branch}
		\Else \label{simple:smalldeg}
		\State find a minimum Vertex Cover $U$ of $G$
		\State \Return  $S=\{u\}$  where $u\in U$ is an arbitrary vertex
		\EndIf 
	\end{algorithmic}
	\caption{$\simp(G,x)$}
	\label{algo:simplevc}
\end{algorithm}
We use a simple structural property of \texttt{Vertex Cover}  to derive the   branching step described in \Cref{algo:simplevc}. The idea behind the branching step is that if the maximum degree of a graph $G$ is $2$ or less  then a minimum vertex cover can be found in polynomial time.  If this is the case, the algorithm returns a vertex from this minimum vertex cover. 
Otherwise, for every vertex  $v$  of degree $3$ or more in the graph, it holds that either $v$ or all its neighbors are in the vertex cover. The algorithm returns  either $v$ or $3$ of its neighbors depending on the value of $x$. 

\begin{observation}
	$\simp$ is a branching step for $\vcvd$. 
\end{observation}

In order to design a procedure from a branching step we need an upper bound on the size of the set returned by a branching step. 
\begin{definition}
	We say a branching step $\step$ is of order $\Delta \in \mathbb{N}$ if for every $G\in \cG\setminus \Pi$ and $x\in [0,1]$ it holds that $\abs{\step(G,x)}\leq \Delta$. 
\end{definition}
The branching step $\simp$ returns a set of size at most $3$ for every input, therefore $\simp$ is of order $3$.

We design a  generic $\proc{\delta}{p}$, to which we refer as $\multistep_{\cG,\Pi,\step,\Delta}$, using a branching step $\step$ or order $\Delta$. The procedure gets an hypergraph $G\in \cG$ and a budget $b\in \mathbb{N}$ as its input. The procedure returns a graph $G' \in \cG$  which is attained by removing up to $b$ vertices from  $G$. Besides $G$ and $b$ the procedure also receives  $b$ numbers $x_1,\ldots, x_b \in [0,1]$ which serve as a source of randomness. In each recursive step the procedure invokes the branching step $\step$ with the input graph $G$. The returned set $S$ is removed from the graph $G$ and the budget is reduced by $\abs{S}$ in the recursive call. The stopping condition for the recurrence is that either $b<\Delta$ or $G\in \Pi$. The condition $G\in \Pi$ is necessary as otherwise $G$ is not a valid input for $\step$. The condition $b<\Delta$ is essential to ensure the output $G'$ is attained by removing at most $b$ vertices from $G$.  The pseudo-code of $\multistep_{\cG,\Pi,\step,\Delta}$ is given in \Cref{algo:multistep}. 


\begin{algorithm}
	\begin{algorithmic}[1]
		\Configuration A  family $\cG$ of hypergraphs, an hypergraph property $\Pi$, a branching step $\step$ for $\gpivd$ of order $\Delta\in \mathbb{N}$
		\Input hypergraph $G \in \cG$, budget $b\in \mathbb{N}$ and numbers $x_1,\ldots, x_b \in [0,1]$ (source of randomness)
		\If {$b<\Delta$ or $G\in \Pi$  }
		\State  	\Return $G$ \label{multi:return}
		\Else
			\State $S\leftarrow \step(G, x_b)$
			\State  			\Return $\multistep_{\cG,\Pi,\step,\Delta}(G\setminus S,b-\abs{S}, x_1,\ldots, x_{b-\abs{S}}) \label{multi:step}
			$
		\EndIf
	\end{algorithmic}
	\caption{$\multistep_{\cG,\Pi,\step,\Delta}(G,b, x_1,\ldots, x_b)$}
	\label{algo:multistep}
\end{algorithm} 
The following observation can be easily shown using an inductive argument. 
\begin{observation}
	\label{obs:multistep_removal} For every $G\in \cG$, $b\in \mathbb{N}$ and $x_1,\ldots, x_b\in [0,1]$, there is $D\subseteq V(G)$, $\abs{D}\leq b$ such that $\multistep_{\cG,\Pi,\step,\Delta}(G,b,x_1,\ldots, x_b) \, =\, G\setminus D$. 
\end{observation}
The next observation trivially follow from the fact that a branching step $\step$ must return a non-empty set  and run in polynomial time (see \Cref{def:step}).
\begin{observation}
	\label{obs:multistep_polynomial}  $\multistep_{\cG,\Pi,\step,\Delta}$ is a polynomial time algorithm.
\end{observation}

Let $(X_i) _{i\in \mathbb{N}_{>0}}$ be an infinite sequence of i.i.d uniformly distributed in $[0,1]$. Given $\delta\geq 1$, we use $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot t})$ to denote the algorithm which receive $G\in \cG$ and $t\in \mathbb{N}$ as input, and then returns $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot t},X_1,\ldots, X_b)$. Using \Cref{obs:multistep_removal}  we can show that $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot t})$ satisfies \Cref{prop:first} of \Cref{definition:proc}. 
\begin{lemma}
	Let $G\in \cG$ and $t\in  \mathbb{N}$. Also, let $G' = \multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot t})$. If $\OPT_{(\cG,\Pi)}(G')\leq k$ then $\OPT_{(\cG,\Pi)}(G) \,\leq \, k+\delta \cdot t$. 
\end{lemma} 
\begin{proof}
	By \Cref{obs:multistep_removal} there is a (random) set $D\subseteq V(G)$ such that $\abs{D} \leq \floor{\delta t} \leq \delta \cdot t$ and $G'= G\setminus D$. If $\OPT_{(\cG,\Pi)}(G')\leq k$  then there is $S\subseteq V(G')$ such that $\abs{S}\leq k$ and $G'\setminus S\in \Pi$. Therefore, $\abs{S\cup D} \leq k+ \delta \cdot t$ and $G\setminus (S\cup D) = G'\setminus S \in \Pi$. That is, $S\cup D \in \sat_\Pi(G)$. Therefore~$\OPT_{(\cG,\Pi)}(G) \,\leq \, k+\delta \cdot t$. 
\end{proof}


\subsection{Success Probability} 
Our objective is to show that $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot t})$  is a $\proc{\delta}{p}$ for some $p$. Towards this end we define a function $Q_{\cG,\Pi,\step,\Delta}:\cG\times \mathbb{N}\times \mathbb{Z} \rightarrow [0,1]$ such  that $Q_{\cG,\Pi,\step,\Delta}(Q,b,t)$ is the probability that the optimum of $\multistep_{\cG,\Pi,\step,\Delta}(G,b,X_1,\ldots, X_b)$ is smaller than the optimum of $G$ by $t$ or more, or alternatively is $0$.  Formally,  we define 
	\begin{equation}
		\label{eq:Qdef}
Q_{\cG,\Pi,\step,\Delta}(G,b,t) \,=\, \begin{cases} \Pr\left(\,\OPT(\multistep_{\cG,\Pi,\step,\Delta}(G,b,X_1,\ldots, X_b)) \,\leq\, \max\left\{ 0, \OPT(G)-t\right\} \,\right) &t\geq 0\\
	0 &t<0\end{cases}
\end{equation}
for every $G\in \cG$, $b\in \mathbb{N}$ and $t\in \mathbb{Z}$. 
We sometimes use $Q$ instead of $Q_{\cG,\Pi,\step,\Delta}$ in case   ${\cG,\Pi,\step,\Delta}$ are known by context. The following lemma connects between $Q$ and the value of $p$.
\begin{lemma}
	\label{lem:lim_to_proc}
	Let $\delta\geq 0$ and define \begin{equation}
		\label{eq:M_def} M\,=-\,\liminf_{t\rightarrow \infty} \frac{1}{t} \inf_{G\in \cG}  \ln \left(Q_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot  t} ,t) \right).
		\end{equation} Then for every $\eps>0$ it holds that $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta \cdot t}))$ is a $\proc{\delta}{p}$ where $p=\exp(-M-\eps)$.  
 \end{lemma}
 \begin{proof}
 	By the definition of $M$ there is $T>0$ such that for every $t\geq T$ it holds that 
 	\begin{equation}  
 		\label{eq:Qliminf}
 		\frac{1}{t} \inf_{G\in \cG}  \ln \left(Q_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot  t} ,t) \right) \geq -M-\eps.
 		\end{equation}
 	
 	Let $G\in \cG$ and $t\geq T$. Also, let $G'=\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot t},X_1,\ldots, X_{\floor{\delta \cdot t}})$ and assume $G$ has a solution of size $k$. Therefore,
 	$$
 	\begin{aligned}
 	\Pr&\left(\,\OPT(G')\,\leq\, \max\{ 0,\, k-t\} \right)  \,\geq\, 	\Pr\left(\,\OPT(G')\,\leq\, \max\{ 0,\, \OPT(G)-t\} \right) \\
 	&=\,\Pr\left(\,\OPT(\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot t},X_1,\ldots, X_{\floor{\delta \cdot t}}))\,\leq\, \max\{ 0,\, \OPT(G)-t\} \right) \\
 	&=\, Q_{\cG,\Pi,\step,\Delta}(G, \floor{\delta\cdot t},t)\\
 	&\geq \,\left(\exp\left(-M-\eps\right)\right)^t\\
 	&= \, p^t,
 	\end{aligned}
 	$$ 
 	where the second equality follows from the definition of $Q_{\cG,\Pi,\step,\Delta}$ \eqref{eq:Qdef} and the last inequality follows form \eqref{eq:Qliminf}. Overall, we showed that $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta \cdot t}))$ is a $\procext{\delta}{p}{1}{T}$, and is therefore a $\proc{\delta}{p}$. 
 \end{proof}


\subsection{Composite Recurrences}
By \Cref{lem:lim_to_proc} it follows that  $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot t})$ is a $\proc{\delta}{p}$,  where $p$ is arbitrarily close to $\exp(-M)$ and $M$ is as defined in \eqref{eq:M_def}. This leads us to the challenge of calculating  the value of $M$. We do so in two steps. In the first provide lower bound $Q_{\cG,\Pi,\step,\Delta}$ using a recurrence relations. The second steps uses the mathematical machinery developed in \cite{KulikS2020} to attain a lower bound for the recurrence.

We begin with the special case of  $\simp$, where we can provide a characterization for the difference $\OPT(G\setminus R)-\OPT(G)$ and size of the set $R$, where $R$ is the output of $\simp(G,X)$. 
\begin{lemma}
	\label{lem:simp_basic}
Let $G\in \vcG\setminus \vcPi$ and let $X\in [0,1]$ be a uniformly distributed random variable. 
Also let $R=\simp(G,X)$ be the random set returned by $\simp$. Then, one of the following holds.
\begin{itemize}
	\item There is $S_1 \subseteq V(G)$ such that $\abs{S_1}=1$, $\OPT(G\setminus S_1) \leq \OPT(G) -1$ and $\Pr(R= S_1 )=1$.
	\item There are $S_1, S_2\subseteq V(G)$ such that $\abs{S_1}=1$, $\abs{S_2} =3$, $\OPT(G\setminus S_1) \leq \OPT(G)-1$, $\Pr(R= S_1)=\gamma$ and $\Pr(R = S_2)=1-\gamma$. 
	\item There are $S_1, S_2\subseteq V(G)$ such that $\abs{S_1}=1$, $\abs{S_2} =3$, $\OPT(G\setminus S_2) \leq \OPT(G)-3$, $\Pr(R= S_1)=\gamma$ and $\Pr(R = S_2)=1-\gamma$. 
\end{itemize}
\end{lemma}
Observe that the probabilities in \Cref{lem:simp_basic} are taken over the probability space defined by $X$. The sets $S_1$ and $S_2$ are deterministic given $G$. Finally, note that second and third bullets provide different guarantees. The second bullet ensure $\OPT(G\setminus S_1) \leq \OPT(G)-1$ while the third stipulates that  $\OPT(G\setminus S_2) \leq \OPT(G)-3$.
\begin{proof}[Proof of \Cref{lem:simp_basic}]
Consider the following cases.
\begin{itemize}
	\item The maximal vertex degree in $G$ is $2$ or less. In this case $\simp(G,X)$ finds a minimum vertex cover $U$ of $G$ and returns $S=\{u\}$ where $u$ is an arbitrary vertex in $U$. Observe that the set  $U$ and vertex $u$ are deterministic given  $G$. Thus, we can define $S_1=\{u\}$. It holds that $\abs{S_1}=1$, $\Pr(R=S_1)=1$ and $\OPT(G\setminus S_1)  \leq \OPT(G)-1$ since $U\setminus \{u\}$ is a vertex cover of $G\setminus \{u\}$. That is, in this case the condition in the first bullet holds.
	\item There is a vertex of degree $3$ or more in $G$. In this case, let $v$ be the vertex selected in \Cref{simple:v} of \Cref{algo:simplevc}, and let $N$ be its three neighbors selected in step \Cref{simple:N}.  Define $S_1 =\{v\}$ and $S_2=N$. Therefore $\abs{S_1}=1$ and $\abs{S_2}=3$. Also, by the logic in \Cref{simple:branch} it holds that 
	$
	\Pr(R=S_1) = \Pr(X\leq \gamma )=\gamma
	$ and $\Pr(R=S_2) = \Pr(X> \gamma )=1-\gamma$.  Finally, let $U$ be a minimum vertex cover of $G$. We consider two sub-cases.
	\begin{itemize}
		\item $v\in U$. Therefore $U\setminus \{v\}$ is a vertex cover of size $\OPT(G)-1$ of $G\setminus \{v\}=G\setminus S_1$. Thus $\OPT(G\setminus S_1) \leq \OPT(G)-1$.  Overall, we showed the condition in the second bullet holds.
		\item $v\notin U$. Since $U$ is a vertex cover it must be that $N\subseteq U$. Therefore $U\setminus N$ is a vertex cover of $G\setminus N = G\setminus S_2$. Hence $\OPT(G\setminus S_2) \leq \OPT(G)-3$.   That is, we showed the third bullet holds. 
	\end{itemize}
\end{itemize}
\end{proof}

We use the shorthand $Q_{\VC} = Q_{\vcG,\vcPi,\simp,3}$, that is,  the function defined in \eqref{eq:Qdef} with respect to \texttt{Vertex Cover}  and the branching step $\simp$ of order $3$. 
We can use \Cref{lem:simp_basic} to lower bound $Q_{\VC}$ using a recurrence. Define, 
\begin{equation}
	\label{eq:simple_q_def}
	\begin{aligned} 
		q(b,t) \, &=\, \min \begin{cases}
			\gamma \cdot q(b-1,t-1) + ~(1-\gamma)\cdot q( b-3,t) \\
			\gamma \cdot q (b-1,t)~~~~~ + ~(1-\gamma)\cdot q(b-3,t-3)\\
			q(b-1,t-1)
		\end{cases}\\
		q(b,t) \,&=\,   0~~~~~~~~\forall b<0, t\in \mathbb{Z}\\
		q(b,t) \,&=\,  1~~~~~~~~\forall b\geq 0, t\leq 0
	\end{aligned}
\end{equation}
We observe the recurrence in \eqref{eq:simple_q_def} has already been studied in \cite{KulikS2020}.  The following lemma can be easily proven using \Cref{lem:simp_basic} and an inductive argument. 
\begin{lemma}
	\label{lem:simple_rec}
	For every graph $G$, $b\in \mathbb{N}$ and $t\in \mathbb{Z}$ it holds that $Q_{\VC}(G,b,t)\geq q(b-3,t)$ where $q$ is the function defined in \eqref{eq:simple_q_def}.
\end{lemma}
The lemma will be later proven as a special case of \Cref{lem:Qtoq} which we prove later in this section.  
Similarly to the way we associated the recurrence defined in \eqref{eq:simple_q_def} with $Q_{\VC}$ and $\simp$, we associate recurrences with other branching steps. Towards this end we use the abstract concepts of {\em terms} and  {\em signature}.

Let $r\in \mathbb{N}_{>0}$. We say a vector $\bgam\in \mathbb{R}_{\geq 0}^r$  is a {\em distribution} if $\sum_{i=1}^{r} \bgam_i = 1$. 
\begin{definition}[term] Let $r\in \mathbb{N}_{>0}$. A {\em term} is a triplet $(\bb,\bt,\bgam)$ such that $\bb\in \mathbb{N}^r_{> 0}$, $\bt\in \mathbb{N}^r_{\geq 0} \setminus \{0\}$, $\bgam \in \mathbb{R}_{> 0}^{r}$ and $\bgam$ is a distribution.    We say $r$ is the {\em length} of the term $(\bb,\bt,\bgam)$. 
\end{definition}
\begin{definition}[signature]
	\label{def:signature}
	Let  $\terms = \{(\bb^j,\bt^j,\bgam^j)~|~j\in[N]\}$ be a subset of $N\in \mathbb{N}_{>0}$ terms  such that $(\bb^j,\bt^j,\bgam^j)$ is of length $r_j$ and let $\step$ be a branching step for $\gpivd$. Additionally, let $X\in [0,1]$ be a random variable uniformly distributed on $[0,1]$.
	We say that $\terms$ is a {\em signature} of $\step$ if for every $G\in \cG\setminus \Pi$ there is $j\in [N]$ and sets $S_i\subseteq V(G)$ for every $i\in [r_j]$ such that
	\begin{itemize}
		\item $\abs{S_i} =\bb^j_i$ for every $i\in [r_j]$.
		\item $\OPT_{(\cG,\Pi)} (G\setminus S_i) \leq \OPT_{(\cG,\Pi)} (G)- \bt^j_i $ for every $i\in [r_j]$.
		\item $\Pr(\step(G,X) = S_i)=\bgam^j_i$ for every $i\in [r_j]$.
	\end{itemize}
\end{definition}
Using \Cref{def:signature} we can obtain a compact form of \Cref{lem:simp_basic}. 
\begin{lemma}
	\label{lem:simp_sig}
	Define 
	\begin{equation}
		\label{eq:simple_terms}
		\terms_{\VC,\gamma} ~=~\{ ((1), (1), (1)), ~( (1,3), (1,0), (\gamma,1-\gamma)) ,~( (1,3), (0,3), (\gamma,1-\gamma))\}.
		\end{equation}
	Then $\terms_{\VC,\gamma}$ is a signature of $\simp$. 
\end{lemma}
\Cref{lem:simp_sig} follows immediately from \Cref{lem:simp_basic} and \Cref{def:signature}. We also associate terms with recurrences.

\begin{definition}[Composite Recurrence]
	\label{def:composite}
		Let  $\terms = \{(\bb^j,\bt^j,\bgam^j)~|~j\in[N]\}$ be a set of $N\in \mathbb{N}_{>0}$ terms  such that $(\bb^j,\bt^j,\bgam^j)$ is of length $r_j$.
	   The {\em composite recurrence} of $\{ (\bb^j, \bt^j, \bgam^j)~|~j\in [N]\}$  is the function $q:\mathbb{Z}\times \mathbb{Z} \rightarrow [0,1]$ defined by the recurrence 
	\begin{equation}
		\label{eq:composite}
		\begin{aligned} 
			q(b,t) \, &=\, \min_{j\in [N] } \sum_{i=1}^{r_j} \bgam^j_i\cdot q(b-\bb^j_i, t-\bt^j_i)\\
			q(b,t) \,&=\,   0~~~~~~~~\forall b<0, t\in \mathbb{Z}\\
			q(b,t) \,&=\,  1~~~~~~~~\forall b\geq 0, t\leq 0
		\end{aligned}
	\end{equation}
\end{definition}
In particular, it can be easily observed that the function $q$ defined in \eqref{eq:simple_q_def} is the composite recurrence of $\terms_{\VC,\gamma}$ \eqref{eq:simple_terms}. The following lemma generalizes \Cref{lem:simple_rec} to arbitrary branching steps.
\begin{lemma}
	\label{lem:Qtoq}
	Let $\step$ be a branching step of order $\Delta$ for $\gpivd$, and let $\terms$ be a signature of $\step$. Then $Q_{\cG,\Pi,\step,\Delta} (G, b,t) \geq q(b-\Delta, t)$ for every $G\in \cG$, $b\in \mathbb{N}$ and $t\in \mathbb{Z}$, where~$q$ is a the composite recurrence of $\terms$. 
\end{lemma} 
\begin{proof}
	Denote 	  $\terms = \{(\bb^j,\bt^j,\bgam^j)~|~j\in[N]\}$ where  $N\in \mathbb{N}_{>0}$ and  $(\bb^j,\bt^j,\bgam^j)$ is a term of length $r_j$ for every $j\in [N]$.
	We use $Q=Q_{\cG,\Pi,\step,\Delta}$ and $\multistep_{\cG,\Pi,\step,\Delta}=\multistep$ throughout the proof. 
	We show by induction on $b\in \mathbb{N}$ that $Q(G,b,t)\geq q(b-\Delta,t)$ for every $G\in \cG$ and~$t\in \mathbb{Z}$. 
\paragraph{base case $0\leq b< \Delta$:}  consider $0\leq b< \Delta$ and let $G\in \cG$ and $t\in \mathbb{Z}$.   Since $b-\Delta<0$, by \eqref{eq:composite} we have
$$
q(b-\Delta,t )\,=\, 0\, \leq Q(G,b,t). 
$$
Hence the induction hypothesis holds for $0\leq b<\Delta$. 

\paragraph{induction step:} Let $b\geq \Delta$ and  assume $Q(G,b',t) \geq q(b'-\Delta,t)$ for every  $0\leq b'<b$, $G\in \cG$ and $t\in \mathbb{Z}$. 
Let $t\in \mathbb{Z}$  and $G\in \cG$. Consider the following cases. 
\begin{itemize}
	\item If $t\leq 0$ then $Q(G,b,t) =1\geq q(b,t)$ as $q(b,t)\in [0,1]$.
	\item   
	 If $G\in \Pi$ then $\multistep(G,b,X_1,\ldots,X_b) = G\in \Pi$ (\Cref{multi:return} in \Cref{algo:multistep}), thus $$\OPT(\multistep(G,b,X_1,\ldots,X_b))=0$$
	 and 
	 $Q(G,b,t) =1\geq q(b,t)$ as $q(b,t)\in [0,1]$.
	 \item If $G\notin \Pi$ and $t>0$ then $\multistep(G,b,X_1,\ldots, X_b) = \multistep(G\setminus R, b-|R|, X_1,\ldots, X_{b-\abs{R}} )$ where $R = \step(G, X_b)$ (see \Cref{multi:step}). Since $\terms$ is a signature of $\step$ there are $j\in [N]$ and $S_1,\ldots, S_{r_j}\subseteq V[G]$ such that $\abs{S_i} = \bb^j_i$, $\OPT(G\setminus S_i) \leq \OPT(G)-\bt^j_i$ and $\Pr(R=S_i) = \bgam^j_i$ for every~$i\in [r_j]$.
	 Denote $$G' \,=\, \multistep(G ,b,X_1,\ldots, X_{b}) \,=\, \multistep(G\setminus R ,b-\abs{R},X_1,\ldots, X_{b-\abs{R}})$$ and
	 \begin{equation}
	 	\label{eq:Gprimei_def}
	 	G'_i \,=\, \multistep(G\setminus {S_i},b-\abs{S_i},X_1,\ldots, X_{b-\abs{S_i}}).\end{equation}Observe that $ G'=G'_i$ in case $R=S_i$. 
	  Therefore,
	 \begin{equation}
	 	\label{eq:Qtoq1}
	 \begin{aligned}
	 	Q&(G,b,t)\,=\,\Pr\left(\,\OPT(\multistep(G,b,X_1,\ldots, X_b)) \,\leq\, \max\left\{ 0, \OPT(G)-t\right\} \,\right) \\
	&=\, \sum_{i=1}^{r_j } \Pr(R=S_i)\cdot \Pr\left(\,\OPT(G') \,\leq\, \max\left\{ 0, \OPT(G)-t\right\} \,\middle|\,R=S_i \right) \\
	&=\, \sum_{i=1}^{r_j }\bgam^j_i\cdot \Pr\left(\,\OPT(G'_i) \,\leq\, \max\left\{ 0, \OPT(G)-t\right\} \,\middle|\,R=S_i \right) \\
	&=\, \sum_{i=1}^{r_j }\bgam^j_i\cdot \Pr\left(\,\OPT(G'_i) \,\leq\, \max\left\{ 0, \OPT(G)-t\right\}  \right)\\
	&\geq \,\, \sum_{i=1}^{r_j }\bgam^j_i\cdot \Pr\left(\,\OPT(G'_i) \,\leq\, \max\left\{ 0, \OPT(G\setminus S_i)-(t-\bt^j_i)\right\}  \right).
	 	 \end{aligned}
	 \end{equation}
	 The first first equality is by the definition of of $Q$, and the second equality follows from the law of total probability. The third equality holds as $G'=G'_i$ in case $R=S_i$ and $\Pr(R=S_i) = \bgam^j_i$. The forth equality holds as $G'_i$ is independent of $R$- observe that $G'_i$ is a function of $X_1,\ldots, X_{b-\abs{S_i}}$ while $R$ is a function $X_b$. 
	 	Finally, the inequality holds as $\OPT(G\setminus S_i) \leq\OPT(G)-\bt^j_i$. Furthermore, by \eqref{eq:Gprimei_def}  we have 
	 	\begin{equation}
	 		\label{eq:Qtoq2}
	 	\begin{aligned}
	 	&\Pr\left(\OPT(G'_i) \,\leq\, \max\left\{ 0, \OPT(G\setminus S_i)-(t-\bt^j_i)\right\}  \right)\\
	 	=\,& \Pr\left(\OPT(\multistep(G\setminus S_i, b-\abs{S_i},X_1,\ldots, X_{b-\abs{S_i}})) \,\leq\, \max\left\{ 0, \OPT(G\setminus S_i)-(t-\bt^j_i)\right\}  \right)\\
	 	=\,& Q(G\setminus S_i, b-\abs{S_i} , t-\bt^j_i)\\
	 	=\,& Q(G\setminus S_i, b-\bb^j_i , t-\bt^j_i)\\
	 	\geq \,& q(b-\bb^j_i- \Delta , t-\bt^j_i),
	 	\end{aligned}
	 	\end{equation}
	 	here	the second equality follows from the definition of $Q$ in \eqref{eq:Qdef}, the third equality holds as $\abs{S_i}=\bb^j_i$, and the inequality follows from the induction hypothesis. 
	 	
		By \eqref{eq:Qtoq1} and \eqref{eq:Qtoq2} we have 
	$$
	 	\begin{aligned}
	 		Q&(G,b,t)\,
	 		\geq \, \sum_{i=1}^{r_j }\bgam^j_i\cdot \Pr\left(\,\OPT(G'_i) \,\leq\, \max\left\{ 0, \OPT(G\setminus S_i)-(t-\bt^j_i)\right\}  \right)\\
	 		&\geq \,\sum_{i=1}^{r_j }\bgam^j_i\cdot q(b-\bb^j_i - \Delta, t-\bt^j_i )\\
	 		&\geq \,\min_{j'=1}^{N} \sum_{i=1}^{r_{j'} }\bgam^{j'}_i\cdot q(b-\bb^{j'}_i - \Delta, t-\bt^{j'}_i )\\
	 		&=\, q(b-\Delta,t),
	 	\end{aligned}
	$$
	where the last equality holds as $q$ is the composite recurrence of $\terms$ (see \eqref{eq:composite}). 
\end{itemize}
Overall we showed that $Q(G,b,t)\geq q(b-\Delta, t)$ in all cases, which completes the induction step and the proof of the lemma. 
\end{proof}

Assume $\step$ is a branching step for $\gpivd$ with a signature $\terms$. Then by \Cref{lem:Qtoq} we have, 
\begin{equation}
	\label{eq:Qtoq}
\liminf_{t\rightarrow \infty} \frac{1}{t} \inf_{G\in \cG}  \ln \left(Q_{\cG,\Pi,\step,\Delta}(G,\floor{\delta\cdot  t} ,t) \right) \, \geq\, \liminf_{t\rightarrow \infty} \frac{1}{t} \ln q(\floor{\delta \cdot t}-\Delta, t),
\end{equation}
where $q$ is the composite recurrence of $\terms$.
Thus, if we show that $\liminf_{t\rightarrow \infty} \frac{1}{t} \ln q(\floor{\delta \cdot t}-\Delta, t) \geq -M$, by \Cref{lem:lim_to_proc}, we get that $\multistep$ is a $(\delta, p)$-procedure for $p=\exp(-M-\eps)$ and every $\eps>0$. 

\subsection{Branching Numbers}
\label{sec:numbers}
 We  use the mathematical machinery developed in \cite{KulikS2020} to compute the right hand term in \eqref{eq:Qtoq}. The machinery associated a {\em critical ratio} and {\em branching numbers} with terms. We first review the definitions from \cite{KulikS2020}. 

\begin{definition}[Critical Ratio]
	Let $(\bb, \bt, \bgam)$ be a term of length $r$. 
	The {\em critical ratio} of  $(\bb, \bt, \bgam)$ is 
	$$
	\begin{aligned}\critical(\bb,\bt,\bgam) \,&=\, \min \left\{ \frac{\bb_i}{\bt_i} ~\middle|~i\in [r], \bt_i \neq 0\right \}\\
		&=\, \min \left\{  \delta>0 \,\middle|\,\exists \blam\in \mathbb{R}^r_{\geq 0}\,:~\blam \cdot \bb \leq \delta \cdot \blam\cdot \bt \textnormal{ and $\blam$ is a distribution}\right\}. 
		\end{aligned}
	$$
\end{definition} 

\begin{definition}[Branching Numbers]
	\label{def:numbers}
	Let $(\bb, \bt, \bgam)$ be a term of length $r$ and let $\delta> \critical(\bb, \bt ,\bgam)$.  The  {\em$\delta$-branching number} of  the term $(\bb, \bt, \bgam)$ is 
	\begin{equation}
		\label{eq:branching_numbers}
		M\,=\, \min \left\{  \frac{1}{\blam\cdot \bt} \cdot \D{\blam}{\bgam} \,\middle|\, \blam\in \mathbb{R}^r_{\geq 0}\,:~\blam \cdot \bb \leq \delta \cdot \blam \cdot \bt, \textnormal{ and $\blam$ is a distribution}\right\}.
	\end{equation}
\end{definition}
It was shown in \cite{KulikS2020}  that the optimization problem described in \eqref{eq:branching_numbers} is {\em quasi-convex}, and therefore the $\delta$-branching number of a term $(\bb,\bt,\bgam)$ can be computed efficiently. We add additional details about this computation towards the end of this section \ariel{TBD}.

We extend the definitions of critical ratio and branching numbers to sets of terms.
\begin{definition}[Critical Ratio for Sets] 
Let $\terms$ be a finite set of terms. The {\em critical ratio} of $\terms$ is $\critical(\terms) = \max \{\critical(\bb,\bt,\bgam)~|~(\bb,\bt,\bgam) \in \terms\}$.
\end{definition} 
That is, the critical ratio of a set of terms is the maximal critical ratio of a term in the set. Similarly, we similarly extend the definition of $\delta$-branching numbers.
\begin{definition}[Branching Numbers for Sets]
	\label{def:set_numbers} Let $\terms$ be a finite set of terms and $\delta>\critical(\terms)$. The $\delta$-branching numbers of $\terms$, is the maximum $\delta$-branching number of a term in $\terms$. 
\end{definition}
The is, if $\terms= \{ (\bb^j,\bt^j,\bgam^j)\,|\,j\in[N]\}$ is a set of $N\in \mathbb{N}_{>0}$ terms and $M_j$ is the $\delta$-branching number of $(\bb^j,\bt^j,\bgam^j)$, then the branching number of $\terms$ is $\max_{j\in [N]} M_j$. 

The main theorem in \cite{KulikS2020} is the following. 
\begin{theorem}	\label{thm:KS}
	Let $\terms$ be a finite set of terms and 
	Let $q$ be the composite recurrence of $\terms$. Also let  $\delta > \critical(\terms)$ and let $M$ be the $\delta$-branching number of $\terms$. Then 
	$$
	\lim_{t\rightarrow \infty} \frac{1}{t}\cdot \ln  q\left( \floor{\delta\cdot t}, t\right)\,=\,-M
	$$
\end{theorem}
Intuitively, \Cref{thm:KS} implies that $q(\floor{\delta \cdot t}, t) \approx  \left(\exp\left(-M\right)\right)^T$.
We  use a minor adaption of \Cref{thm:KS} which provides the limit we are looking for.
\begin{restatable}{lemma}{adaptks}
	\label{lem:adaptKS}
Let $\terms$ be a finite set of terms and 
let $q$ be the composite recurrence of $\terms$. Also let  $\delta > \critical(\terms)$ and let $M$ be the $\delta$-branching number of $\terms$. Then for every $\xi\in \mathbb{N}$ it holds that 
	$$
	\lim_{t\rightarrow \infty } \frac{1}{t}\cdot \ln  q\left( 
	\floor{\delta \cdot t -\xi }, t \right)\,=\,- M
	$$
\end{restatable} 
We give the proof of \Cref{lem:adaptKS} in \Cref{app:vertex_cover}, and uses \Cref{thm:KS} as a black-box. 

We use \Cref{lem:adaptKS} to evaluate the success probability of $\multistep_{\cG,\Pi,\step,\Delta}$. 
\begin{lemma}
	\label{lem:multi_success}
	Let $\step$ be a branching step of order  $\Delta$ and let $\terms$ be  a signature of $\step$.
	Also, let  $\delta >0$ such that $\delta > \critical(\terms)$ and let $M$ be the $\delta$-branching number of $\terms$. Then for every $\eps>0$ it holds that $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta \cdot t})$ is a $\proc{\delta}{p}$ where $p=\exp(-M-\eps)$. 
\end{lemma}
\begin{proof}

Let $q$ be the composite recurrence of $\terms$. By \Cref{lem:adaptKS} it holds that 
	$$
\lim_{t\rightarrow \infty } \frac{1}{t}\cdot \ln  q\left( 
\floor{\delta \cdot t -\Delta }, t \right)\,=\,- M.
$$
Using the above equality  together with \Cref{lem:Qtoq} we get
$$
\lim_{t\rightarrow \infty} \frac{1}{t} \inf_{G\in \cG} \ln \left( Q (G,\floor{\delta \cdot t}, t)\right) \, \geq \,
\lim_{t\rightarrow \infty } \frac{1}{t}\cdot \ln  q\left( 
\floor{\delta \cdot t -\Delta }, t \right)\,=\,- M,
$$
where  $Q=Q_{\cG,\Pi,\step,\Delta}$.  Therefore, by \Cref{lem:lim_to_proc} it holds that $\multistep_{\cG,\Pi,\step,\Delta}(G,\floor{\delta \cdot t})$ is a $\proc{\delta}{p}$ for $p=\exp(-M-\eps)$ for every $\eps>0$. 
\end{proof}

\Cref{lem:multi_success} can be used to attain a $\proc{\delta}{p}$ using $\multistep$ and the branching step $\simp$.
\begin{corollary}
	For every $\delta>1$, $\gamma\in (0,1)$ and $\eps>0$  there is a $\proc{\delta}{p}$ for \textnormal{\texttt{Vertex Cover}} where $p=\exp(-M-\eps)$ and $M$ is the $\delta$-branching number of $\terms_{\VC,\gamma}$. 
\end{corollary}

Furthermore, by \Cref{lem:multi_success} and \Cref{thm:beta_approx} we get the following.
\begin{corollary}
	\label{cor:advanced_branching_d}
	Suppose there exists a branching set $\step$  with signature $\terms$ for $\sgpivd$. Furthermore, assume there is a parameterized $\alpha$-approximation for $\sgpivd$ in time $c^k\cdot n^{\Oh(1)}$ for some $\alpha, c\geq 1$. Let $\beta>1$ and $\delta \in \params(\alpha,\beta)$ and assume $\delta>\critical(\terms)$. Then there is a parameterized $\beta$-approximation algorithm for $\sgpivd$ which runs in time 
	$$d^k\cdot n^{\Oh(1)},$$
	where 
	$$d= \exp\left( \frac{(\delta- \beta)\cdot \ln(c )+(\beta-\alpha)\cdot M}{\delta -\alpha}	
	\right) $$
	and $M$ is the $\delta$-branching number of $\terms$.
\end{corollary}



\subsection{Improved Branching Step for Vertex Cover} 
\label{sec:improved_vc}
\ariel{The subsection should be edited to the notion of branching steps}
We can further improve the running time of \Cref{algo:simplevc} by using a more refined point of view. Consider an arbitrary graph $G\in \cG$ and $v\in V$ of degree {\bf exactly}  $3$. Also, let $\OPT$ be a vertex cover of $\OPT$ (that is, $\OPT\in \sat_\Pi(G)$). The idea behind the randomized branching in \Cref{algo:simplevc} is that either $v\in \OPT$ or $N(v)\subseteq \OPT$.  In case $v\in \OPT$, then with probability $\gamma$ the algorithm adds $v$ to $S$ and reduces the minimum vertex cover size in $G\setminus S$ by $1$, and with probability $(1-\gamma)$ the algorithm adds $N(v)$ to the solution. The analysis assumed the latter case does no incur any reduction to the minimum vertex cover size of $G\setminus S$. This analysis is not tight. Since $v$ of degree $3$, it can be easily observe that $\OPT\setminus \{v\}$ is a vertex cover of $G\setminus N(v)$, thus adding $N(v)$ to $S$ decreased the minimum vertex cover size of $G\setminus S$ by $1$ (or more). \Cref{algo:improVC} leverages this observation to attain better running times. 

\begin{algorithm}
	\begin{algorithmic}[1]
		\Configuration $\Delta\in \mathbb{N}$, $\Delta>3$ and numbers $\gamma_d \in (0,1)$ for every integer $3\leq i\leq \Delta$.
		\Input graph $G \in \mathcal{G}$, integer $b \geq 0$
		\State {\bf if} $G$ has no edges or $b< \Delta$ {\bf then} \Return $G$ \label{imp:initial}
		\If {there is $v\in V[G]$ with $\deg_{G}(v)\geq 3$\label{imp:v}} 
		\State define $d= \min\left\{ \deg_G(v), \Delta\right\}$
		\State let $N$ be $d$  of the neighbors of $v$ \label{imp:N}
		\State set $S\leftarrow \{v\}$ with prob $\gamma_d$  and  $S\leftarrow N$ with probability $1-\gamma_d$
		\label{imp:branch}
		\Else \label{imp:smalldeg}
		\State find a minimum Vertex Cover $U$ of $G$
		\State set $S=\{u\}$  where $u\in U$ is an arbitrary vertex
		\EndIf 
		\State  		
		\label{imp1:return}
		\Return $\imp(G\setminus S, b-|S| )$
	\end{algorithmic}
	\caption{$\imp(G,b)$}
	\label{algo:improVC}
\end{algorithm}

Like \Cref{algo:simplevc},
\Cref{algo:improVC} uses random branching which either adds $v$ or a subset of neighbors of $v$ to $S$. Unlike \Cref{algo:simplevc}, in case the degree of $d$ is less than a configuration parameter $\Delta$, the algorithm either selects $v$ or {\em all} its neighbors to $S$. Also, the probability by which $v$ is selected to $S$ is $\gamma_d$, which depends on the degree of $v$.  A main benefit of the algorithm (in comparison to \Cref{algo:simplevc}) is that even an incorrect randomized branching (selecting $N(v)$ to $S$ while $N(V)$ may not intersect with the optimum), can still reduce the minimum vertex cover size of $G\setminus S$. 

We first observe that \Cref{algo:improVC} always returns a graph $G'$ for which there is $X\subseteq V[G]$, $\abs{X}\leq b$ such that $G'=G\setminus X$. It therefore holds that if $G'$ has a vertex cover $Y$  (solution) of size $k$, then $X\cup Y$  is a vertex cover of $G$ of size $k+b$. We use $\imp(G,\floor{\delta,t})$ to denote the algorithm which receives $G\in \cG$ and a number $t$ as an input, and invoke $\imp(G,\floor{\delta,t})$. By the above argument we attain the following observation.
\begin{observation}
	\label{obs:imp_first_prop}
	For any $\delta\geq 1$ it holds that  $\imp(G,\floor{\delta,t})$ satisfies \Cref{prop:first} of \Cref{definition:proc}. 
\end{observation}

As in the analysis of \Cref{algo:simplevc}, for every $G\in \cF$, $b\in \mathbb{N}$ and $t\in \mathbb{Z}$ define 
\begin{equation}
	\label{eq:impQ}
	Q(G,b,t) \defeq \begin{cases}   \Pr\left( \VC(\imp(G,b))\,\leq\, \max\{0, \VC(G)-t\}\right) 
		& t\geq 0\\
		1 & t<0 
	\end{cases},
\end{equation}
as the probability that \Cref{algo:improVC} decreases the minimum vertex cover size of $G$ by $t$ or to $0$. As before, we consider the event  $\VC(\imp(G,b))\,\leq\, \max\{0, \VC(G)-t\}$ as ``success'' of the algorithm.

Consider the following composite recurrence,
\begin{equation}
	\label{eq:imp_q_def}
	\begin{aligned} 
		q(b,t) \, &=\, \min \begin{cases}
			\gamma_d \cdot q(b-1,t-1) + ~(1-\gamma_d)\cdot q( b-d,t-1) & 3\leq d <\Delta  \\
			\gamma_\Delta \cdot q(b-1,t-1) + ~(1-\gamma_\Delta)\cdot q( b-d,t)  \\
			\gamma_d \cdot q (b-1,t)~~~~~ + ~(1-\gamma_d)\cdot q (b-d,t-d)  &3\leq d \leq \Delta \\
			q(b-1,t-1)
		\end{cases}\\
		q(b,t) \,&=\,   0~~~~~~~~\forall b<0, t\in \mathbb{Z}\\
		q(b,t) \,&=\,  1~~~~~~~~\forall b\geq 0, t\leq 0
	\end{aligned}
\end{equation}
It holds that $q$ is a composite recurrence (\Cref{def:composite}). Let $\terms$ be the a set of terms such that~$q$ is the composite recurrence of $\terms$. Note that $\terms$ (and similarly $q$) depend on $\Delta$ and the values $\gamma_3,\ldots, \gamma_\Delta$. We keep this dependency implicit. 
We can lower bound $Q$ in terms of the recurrence $q$. 
\begin{lemma}
	\label{lem:imp_rec}
	For every graph $G$, $b\in \mathbb{N}$ and $t\in \mathbb{Z}$ it holds that $Q(G,b,t)\geq q(b-\Delta,t)$. 
\end{lemma}
A formal proof of \Cref{lem:imp_rec} follows along the lines of the proof of \Cref{lem:simple_rec} given in \Cref{app:vertex_cover}. We omit the formal proofs, but provide the main argument in it.
Consider an execution of the algorithm with the input $G$ and $b$.  Let $\OPT$ to be a minimum size vertex cover of the input graph $G$. Furthermore, assume \Cref{imp:branch} is reached, the let $v$, $N$ and $d$ be as defined in the algorithm.  We consider several case.
\begin{itemize}
	\item $v\in \OPT$ and $d<\Delta$. In this cases $\VC(G\setminus \{v\})=\VC(G)-1$  trivially holds. Furthermore,  $\VC(G\setminus N) =\VC(G\setminus N(v))\leq \VC(G)-1$ since $\OPT\setminus \{v\} \setminus N(v)$ is a vertex cover of $G\setminus N(v)$. Thus, with probability $\gamma_d$ the algorithm selects $S=\{v\}$, and succeeds if the recursive call for $\imp(G\setminus \{v\}, b-1)$ reduces the size of the vertex cover of $G$ by $t-1$, and with probability $1-\gamma_d$ the algorithm selects $S=N(v)$ and succeeds if the recursive call for 
	$\imp(G\setminus N(v), d)$ reduces the size of the vertex cover of $G$ by $t-1$. Following this argument it can be shown that,
	$$Q(G,b,t)\,\geq\, \gamma_d\cdot Q(G\setminus \{v\},b-1,t-1) + (1-\gamma_d)\cdot Q(G\setminus \{v\},b-d,t-1).$$
	\item $v\in \OPT$ and $d=\Delta$. As in the previous case, $\VC(G\setminus \{v\})=\VC(G)-1$, but we can only use the trivial claim $\VC(G\setminus N)\leq \VC(G)-1$ as some of the neighbors of $v$ may not be in $N$. Therefore, with probability $\gamma_{\Delta}$ the algorithm selects $S=\{v\}$ and in order to succeed the recursive call for $\imp(G\setminus\{v\},b-1)$ only needs to reduce the minimum vertex cover size of $G\setminus \{v\}$ by $t-1$. Also, with probability $(1-\gamma_{\Delta})$ the algorithm selects $S=N$, and to ensure success the recursive call for $\imp(G\setminus N,b-\abs{N})$  has to reduce the minimum vertex cover size of $G\setminus N$ by $t$. Overall, we can show that 
	$$Q(G,b,t)\,\geq\, \gamma_{\Delta}\cdot Q(G\setminus \{v\},b-1,t-1) + (1-\gamma_{\Delta})\cdot Q(G\setminus N,b-\Delta,t).$$
	\item $v\notin \OPT$. In this case it must hold that $N\subseteq N(v) \subseteq \OPT$, and therefore $\VC(G\setminus  N)\leq \VC(G) -\abs{N}$. With probability $1-\gamma_{d}$ the algorithm selects $S=N$ and in order to succeed the recursive call for $\imp(G\setminus N, b-d)$ only needs to further reduce the minimum vertex cover size by $t-d$. With probability $\gamma_d$ the algorithm selects $S=\{v\}$, and in order to succeed the recursive call for $\imp(G\setminus \{v\},b-1)$ needs to reduce the minimum vertex cover size by $t$. By the above argument it can be show that
	$$Q(G,b,t)\,\geq\, \gamma_{d} \cdot Q(G\setminus \{v\},b-1,t) + (1-\gamma_d)\cdot Q(G\setminus N, b-d, t-d).$$
\end{itemize}
The above inequalities can be combined with a simple induction to show \Cref{lem:imp_rec}. 

\begin{lemma}
	Fix $\delta>1$. 
	Let $\Delta\in \mathbb{N}$, $\Delta \geq 3$.
	For every term $t\in \terms$ let $M_t$ be the $\delta$-branching number of the term $t$. Then for every $\eps>0$ it holds that $\imp(G,\floor{\delta \cdot t})$ is a $(\delta,p)$-procedure for vertex cover where $$p = \exp\left( -\max_{t\in \terms} M_t -\eps\right).$$ 
\end{lemma}
\begin{proof}
	\ariel{the proof is in practice a copy paste of the previous proof. We should think of a method to write down a single proof. 
	}
\end{proof}

\subsection{Vertex Cover on Graph with Maximal Degree $3$}
\subsection{$3$-Hitting Set, $3$-path Vertex Deletion}

